Do Large Multimodal Models Solve Caption Generation for Scientific Figures? Lessons Learned from SciCap Challenge 2023

Since the SciCap datasets launch in 2021, the research community has made significant progress in generating captions for scientific figures in scholarly articles. In 2023, the first SciCap Challenge took place, inviting global teams to use an expanded SciCap dataset to develop models for captioning diverse figure types across various academic fields. At the same time, text generation models advanced quickly, with many powerful pre-trained large multimodal models (LMMs) emerging that showed impressive capabilities in various vision-and-language tasks. This paper presents an overview of the first SciCap Challenge and details the performance of various models on its data, capturing a snapshot of the fields state. We found that professional editors overwhelmingly preferred figure captions generated by GPT-4V over those from all other models and even the original captions written by authors. Following this key finding, we conducted detailed analyses to answer this question: Have advanced LMMs solved the task of generating captions for scientific figures?

==> sections/data-split.tex <==
We split the data similar to the format of \textbf{mscoco} dataset. Our dataset contains both ArXiv and ACL. For ArXiv, we split the dataset into training, validation, public test and hidden test set which contain 70\% (333,472 samples), 10\% (47,639 samples), 10\% (47,639 samples) and 10\% (47,639 samples) respectively. For ACL, we removed all the papers that were already published at arXiv. Due to the size of the data, we only use it as an additional training set which contain 26,868 samples. 



==> sections/evaluation-by-domain.tex <==
To conduct an in-depth analysis and comparison of features across different fields, we breakdown the evaluation based on the figures' primary domain, as identified by the first category listed on arXiv. This method aligns with the arXiv Category Taxonomy and separates the figures into eight main domains: Computer Science, Economics, Electrical Engineering and Systems Science, Mathematics, Physics, Quantitative Biology, Quantitative Finance, and Statistics. Out of a total of 47,639 figures, the distribution is as follows: Computer Science with 18,521 figures, Economics with 69, Electrical Engineering and Systems Science with 1,248, Mathematics with 2,316, Physics with 23,668, Quantitative Biology with 499, Quantitative Finance with 266, and Statistics with 1,052 figures. The detailed results are presented in~\Cref{fig:domains-rouge2_scores}.



==> sections/evaluation-by-figuretype.tex <==
Mirroring our analysis of domains, we also perform a thorough review across different figure types, organizing the evaluation into five distinct categories: Node Diagram, Equation, Graph Plot, Scatterplot, and Bar Chart, using the classification model provided by Figureseer~\cite{siegel2016figureseer}. In this context, we follow \dataset~\cite{hsu2021scicap} to exclude Tables due to their fundamental difference from the essence of figures, as well as the 'Others' category for figures that do not fit into any classification. Among a total of 47,639 figures analyzed, there are 7,215 Node Diagrams, 3,192 Equations, 29,276 Graph Plots, 4,161 Scatterplots, and 3,795 Bar Charts. The detailed results are presented in~\Cref{fig:figtype-rouge2_scores}.



==> sections/expend-scicap.tex <==
The main dataset provided for the Challenge is an expanded version of the \dataset~\cite{hsu2021scicap} dataset. It incorporates figures and captions extracted from arXiv papers, covering a wider range of domains and figure types compared to the original \dataset dataset.

This dataset is composed of papers from January 2010 to October 2020. It encompasses eight distinct categories: Computer Science, Economics, Electrical Engineering and Systems Science, Mathematics, Physics, Quantitative Biology, Quantitative Finance, and Statistics.
